Statistical Modeling for Practical Pooled Testing During the COVID-19 Pandemic

Pooled testing offers an efficient solution to the unprecedented testing demands of the COVID-19 pandemic, although with potentially lower sensitivity and increased costs to implementation in some settings. Assessments of this trade-off typically assume pooled specimens are independent and identically distributed. Yet, in the context of COVID-19, these assumptions are often violated: testing done on networks (housemates, spouses, co-workers) captures correlated individuals, while infection risk varies substantially across time, place and individuals. Neglecting dependencies and heterogeneity may bias established optimality grids and induce a sub-optimal implementation of the procedure. As a lesson learned from this pandemic, this paper highlights the necessity of integrating field sampling information with statistical modeling to efficiently optimize pooled testing. Using real data, we show that (a) greater gains can be achieved at low logistical cost by exploiting natural correlations (non-independence) between samples -- allowing improvements in sensitivity and efficiency of up to 30% and 90% respectively; and (b) these gains are robust despite substantial heterogeneity across pools (non-identical). Our modeling results complement and extend the observations of Barak et al (2021) who report an empirical sensitivity well beyond expectations. Finally, we provide an interactive tool for selecting an optimal pool size using contextual information

==> COVID Pooled Testing Draft Paper 2/abstract.tex <==
% !TEX root = main.tex


% Pooled testing offers an appealing and efficient solution to the unprecedented testing demands of the COVID-19 pandemic, potentially at the price of a lower sensitivity and increased costs to implementation. However, assessments of this trade-off typically assume pooled specimens to be \textit{independent and identically distributed} (iid). Yet, in the context of COVID-19, these iid assumptions are often violated: testing done on networks (such as co-workers in an office, students in a dormitory, inmates in a prison) captures correlated (\textit{non-independent}) individuals, while we now know that risk of infection varies substantially across time and individuals (\textit{non-identical}). Neglecting dependencies and heterogeneity may yield inaccurate  estimates of pooled testing efficiency and induce its sub-optimal implementation through a bias in established optimality grids. 

% %This creates a critical need for the fast readjustment of current pool sampling procedures. 
% %As a lesson learned from this pandemic, this paper aims to show that statistical modeling informed by practical constraints can provide useful information to deploy group testing in the novel and unprecedented setting of the COVID-19 pandemic and --- better yet --- to leverage deviations from the standard i.i.d assumptions to further optimize pooling. 
% As a lesson learned from this pandemic, this paper aims to show that the combination of practical field information regarding the logistics of specimen sampling with statistical modeling is crucial in rapidly and accurately optimizing group testing procedures. 
% In particular, we show that (a) greater and more feasible gains can be achieved by exploiting natural correlations (\textit{non-independence}) between samples --- allowing improvements in sensitivity and efficiency up to 30\% and 90\% greater than under iid settings ; and (b) these gains are robust despite substantial heterogeneity across pools (\textit{non identical}). 
% %Due to the tension between statistical and logistical optimality, we focus on the more practical two-stage Dorfman procedure and 
% We use observed data to quantify the impact of correlated sampling processes on several metrics of interest (sensitivity, sensitivity relative to individual testing, average number of test per sample, and missed cases per sample). Our modeling results align with,  complement and extend the empirical observations of \cite{Barak2021} who highlight a sensitivity of pooled sampling beyond expectations on real data. Finally, we provide an interactive tool for selecting an optimal pool size using contextual information.\footnote{The corresponding shiny-app interface is available at: \url{https://homecovidtests.shinyapps.io/Group-testing/}}


Pooled testing offers an efficient solution to the unprecedented testing demands of the COVID-19 pandemic, although with potentially lower sensitivity and increased costs to implementation in some settings. Assessments of this trade-off typically assume pooled specimens are independent and identically distributed. Yet, in the context of COVID-19, these assumptions are often violated: testing done on networks (housemates, spouses, co-workers) captures correlated individuals, while infection risk varies substantially across time, place and individuals. Neglecting dependencies and heterogeneity may bias established optimality grids and induce a sub-optimal implementation of the procedure.\\
\indent As a lesson learned from this pandemic, this paper highlights the necessity of integrating field sampling information with statistical modeling to efficiently optimize pooled testing. Using real data, we show that (a) greater gains can be achieved at low logistical cost by exploiting natural correlations (non-independence) between samples —allowing improvements in sensitivity and efficiency of up to 30\% and 90\% respectively; and (b) these gains are robust despite substantial heterogeneity across pools (non-identical). Our modeling results complement and extend the observations of \citeauthor{Barak2021} who report an empirical sensitivity well beyond expectations. Finally, we provide an interactive tool for selecting an optimal pool size using contextual information\footnote{The corresponding shiny-app interface is available at: \url{https://homecovidtests.shinyapps.io/Group-testing/}}.




==> COVID Pooled Testing Draft Paper 2/acknowledgements.tex <==
We thank Dr. Benjamin Pinsky (Associate Professor of Pathology and Medicine at Stanford University) for sharing data with us and for his feedback on the manuscript. 

==> COVID Pooled Testing Draft Paper 2/conclusion.tex <==
% !TEX root = main.tex

Violations of i.i.d assumptions and high prevalence settings have typically been considered impediments to using pooled testing; however, we demonstrate, mathematically and via simulation, that significant gains can be made in terms of testing efficiency and sensitivity by taking advantage of correlated samples and high probabilities of positive samples. Clustering multiple positive samples in a single pool improves both efficiency (by focusing re-testing in a directed fashion) and sensitivity (by increasing the concentration of viral genetic material). We also investigate the effects of heterogeneity in the input parameters- specifically prevalence and network transmission- on the outcome metrics of interest. We find that our overall findings are robust to heterogeneity. This suggests that these methods can be useful even in real-world settings where precise values of prevalence and network transmission may not be known.\\
\indent For example, at the peak of the pandemic in Alabama in January 2021, pooled samples of size 5 collected from households with symptomatic index cases could have reduced testing needs by 58\%; at that time, the positive test rate in Alabama exceeded 20\%, and greater testing capacity was urgently needed. Pooling in this setting and with this pool size is predicted to have sensitivity far exceeding individual tests, even when accounting for uncertainty in both prevalence and network transmission rates. Even greater savings can be observed in other settings, such as Maine in October 2020, a period when prevalence was low: pooled testing in pools of size 20 would have reduced testing requirements by over 90\% relative to individual testing in both high and low network transmission settings. For moderately high values of network transmission (household transmission with a symptomatic index case and spouses), the sensitivity of this procedure again exceeds individual testing.\\
In conclusion, as a lesson learned from the pandemic, we highlight the importance of "field-aware" statistical modeling and the importance of adaptive models. To develop an actionable response to the pandemic and its unprecedented conditions, it is important to develop statistical model that accurately optimize procedures to the population at hand. This development has to be done in close collaboration with clinicians, to ensure the feasibility and scalability of the proposed solution. Here, we demonstrate that leveraging correlations in specimen collection procedures and incorporating knowledge about local prevalence and network transmission parameters can lead to better informed, logistically-feasible, and adaptive pooled testing.

%In conclusion, this paper focuses on finding a way to leverage correlations in specimen collection procedures, which we estimate can increase test efficacy by X\% and decrease test costs by Y\%.
%In contrast to other papers, we also focus on adding various levels of heterogeneity in our scenarios, which we believe to be more informative.

==> COVID Pooled Testing Draft Paper 2/discussion.tex <==
% !TEX root = main.tex


Pool testing can also be considered as a spectrum: from $p=1$,where we consider individual tests, to $p=\infty$, where we are interested in extremely large pools and in this case, are using pool testing as a monitoring tool (widespread surveillance of the population). In this case , we might not necessarily be interested in the individual samples themselves and perform a two stage Dorfman procedure. Rather, in this section, we investigate how pooled testing can be used as a monitoring tool, and to recover the prevalence level. In particular, we will focus on investigating how PCR can be used quantitatively, rather than qualitatively --- to perform inference.

Suppose that we want to infer the prevalence from group testing.


The probability that the pool tests positive is :
$$ p = 1- (1-\pi)^n $$
We want to infer $\pi$.

If we were to observe $p$ pools the plug in estimator would be:
$$  \bar{Y}_p = 1- (1-\hat{\pi})^n)$$
$$  \hat{\pi} = 1- (1 -\bar{Y}_p)^{1/n} $$

Because we are typically looking at very small probabilities, it might be better to use exact confidence intervals. 

That is, we solve:
$$ \frac{\alpha}{2} \geq \sum_{k=0}^{p\bar{Y}_p} {p \choose p\bar{Y}_p} p_L^{ p\bar{Y}_p} (1-p_L)^{ p- p\bar{Y}_p} \qquad p_L = 1-(1-\hat{\pi}_L)^n$$
$$ \frac{\alpha}{2} \geq \sum_{k=p\bar{Y}_p}^p {p \choose p\bar{Y}_p} p_H^{ p\bar{Y}_p} (1-p_H)^{ p- p\bar{Y}_p} \qquad p_H = 1-(1-\hat{\pi}_H)^n $$

This creates confidence bands that are perhaps a little large (include a plot).


Our other suggestion here is to try to use the quantitative information contained in the Ct value to enrich this. Roughly, if the $C_t$ value is high, it will be more reflective of a low number of samples being positive, and vice versa.

We have:
$$ Y_i = 1\{ C_t \geq T\} $$
Let $m_0$ be the initial quantity of viral material in the initial sample, and $T$ a threshold for declaring the sample as positive:
$$ m^{(0)} 2^{C_t} = T \implies m^{(0)} =  \frac{T}{2^{C_t}} $$
Thus, in the combined sample:
$$ M = \sum_{i=1}^n m^{(0)}_i =  \sum_{i=1}^n \frac{T}{2^{C^t_i}} $$
$$ \implies C_M^t = \frac{\log( \frac{T}{ \sum_{i=1}^n \frac{T}{2^{C^t_i}}})}{\log 2} = \frac{-\log( \sum_{i=1}^n \frac{1}{2^{C^t_i}})}{\log 2} $$


So we transform the problem of inferring the prevalence in:

$$ \text{Find $\pi$ such that: }\qquad \pi = \tetx{argmax}_{\pi} \ell(\pi)  $$

(MLE) of the latent variable model, with:
$$  C_i \sim  \text{Mixture}(0, \text{Weibull) with probability $\pi$} $$
We can probably provide an abacus of sorts: We can get via MCMC simulations the distribution of $C_M^t$for different numbers of positives. And treat $\pi$ as Bernouilli (makes sense for very large pools), and:
\begin{itemize}
    \item We look at all the distributions of $C_M$ that overlap with the observed value (probability of observing that value between $[2.5;97.5]$).
    \item We use the min and max values of the prev of these distributions to infer what the prevalence is.
\end{itemize}

The issue with this procedure is that it is based on a discretization of the space. So it might require a lot of computations? Remains to show that this yields better result than the naive binomial way of doing things. Let's do simulations to check.

==> COVID Pooled Testing Draft Paper 2/heterogeneity.tex <==
% !TEX root = main.tex

So far, our discussion has focused  on situations where the prevalence and the transmission levels are fixed, known quantities.  As such, all the quantities that we have computed are conditional expectations given $\tau, \pi$. However, in practice, these are estimates with associated levels of uncertainty and thus can themselves be modeled  as random variables, whose variability has to be taken into account as we compute metrics of interest. Given the non-linear nature of the model and the wide uncertainty around the value of the network transmission rate (or SAR) $\tau$, it is important to evaluate how much this added variability affects our estimates of the performance of pooled sampling. Uncertainty and heterogeneity are crucial aspects of COVID-19 kinetics that need to be accounted for to ensure accurate  epidemiological predictions  (\cite{cirillo2020tail,cave2020covid,gomez2020mapping,zhang2020evaluating}): most COVID-19 forecasting models --- whether geared towards the prediction of the incidence rate, underascertainment bias, or towards the performance of pooled testing, such as the one considered in this paper ---  are indeed non-linear functions of many unknown and/or highly variable quantities. When solely considering the average rather than accounting for the distributional nature of these variables,  the error can rapidly amplify, and thus needs to be appropriately characterized and controlled (\cite{donnat2021modeling}).  In this section, we (a) show that in the prevalence/SAR regimes that we are considering,  the main driver of the heterogeneity lies in the uncertainty around network transmission and is a function of the behavior of the distribution at the tail, rather than of its variability, (b) highlight ranges of parameters $(n, \pi, \tau)$ which are robust to this heterogeneity, and (c) show via experiments how to construct (and interpret) prediction intervals for the performance of pooled sampling under uncertainty.


\xhdr{Observation 5} \textit{The sensitivity and efficiency (tests per sample) of the alternative model can never be worse than the null model.} This is due to the fact that the (true) effective number of tests per samples can be written as:
$$\eta = \frac{1 +  \mathbb{P}[\sum_{i=1}^n Y_i>0]}{n} =\frac{1}{n} + \frac{1- (1-\pi)^n }{n} =\frac{1}{n} + \pi + o(\pi)$$ in both scenarios. From this formulation we observe that the efficiency is not a function of the network transmission, and depends only on community transmission rates. As such, results on the efficiency are robust for all parameterizations and levels of uncertainty in the value of $\tau$, but will solely depend on the uncertainty for $\pi$. This fact also highlights the necessity of having accurate estimates of the prevalence, tailored to the population at hand in order to correctly optimize pooled testing. In this context, estimates of the prevalence for the sampling population, using hyper-local data and/or additional covariates such as vaccination rates  can be crucial in  further reducing  this uncertainty (\cite{harvard2021,cramer2021evaluation,donnat2021predictive, zhou2020spatiotemporal}).
%The null model provides lower bounds for the network transmission: the efficiency of the pooled testing procedure is indeed identical under both scenarios. 

For the sensitivity, since correlations can only increase the number of positive samples per pool and sensitivity is an increasing function of the $C_t$, the sensitivity can only be improved by taking into account correlations between individuals in the alternative model.


\xhdr{Observation 6} \textit{We can identify settings in which pooled sampling will have worse sensitivity than individual testing.} Since under correlations, the number of positive samples per infected pool is  well approximated by $1 + \text{Binomial}(n-1, \tau)$ (since with 95\% probability, community transmission yields only one infected sample), the number of infected samples can vary quite substantially:
\begin{equation*}
    \begin{split}
    \mathbb{V}_{H_a}[\sum_{i=1}^n Y_i | \sum_{i=1}^n Y_i>0]& = \mathbb{E}[ \mathbb{V}_{H_a}[\sum_{i=1}^n Y_i | \tau, \sum_{i=1}^n Y_i>0]] + \mathbb{V}[ \mathbb{E}_{H_a}[\sum_{i=1}^n Y_i | \tau, \sum_{i=1}^n Y_i>0]]    \\
    & \approx \mathbb{E}[(n-1)\tau(1-\tau)] + \mathbb{V}[ 1 + \tau (n-1)]    \\
      & \approx  (n-1) (n-2) \sigma_{\tau}^2   + (n-1)\mu_{\tau}(1-\mu_{\tau})  \\
    \end{split}
\end{equation*}
where $\mu_{\tau}$ and $\sigma_{\tau^2}$ are respectively the mean and variance of $\tau$.  We can now examine the effect of this variance on the sensitivity.
As seen in the first section, the sensitivity is impacted if the number of positive samples in infected pools falls below 2. This would mean that network transmission only accounts for a single additional infected sample in the pool. 
This event, which has (by property of the binomial) probability equal to  $(n-1) \tau(1-\tau)^{n-2}$ can be deemed highly unlikely as long as it happens with probability less than 0.05. This allows us to solve for regions $\Omega$ of the parameter space for $\tau$ where we expect robust performances of pooled testing, which improve upon individual testing:
\begin{equation*}
    \begin{split}
    \Omega = \{ \tau \in[0,1]: \quad   (n-1) \tau(1-\tau)^{n-2} \leq 0.05 \}.
        \end{split}
\end{equation*}
This allows the user to select a pool size such that, with probability $ 1- \mathbb{P}[\tau \in \Omega]$, the procedure is better than individual testing. Choosing the value of $\eta$ is setting a tolerance threshold, and should be defined by the user.
%  Thus, the result is robust to the choice of uncertainty as long as:
%  $$ \mathbb{P}[\tau \in \Omega] <  \eta,$$
%  where $\eta$ is a tolerance threshold that is chosen by the user.

% \noindent \textbf{Observation 8. } The impact of the variability of $\tau$ on the robustness of the results is a function of the skewness of its left tail. Under Assumption 1  ($\pi n \leq 0.15$), since the probability that more than one sample in the pool is of the order of 1\%,  the number of positive samples in a contaminated pool behaves as a binomial distribution with parameter $\tau$. We consider the following two mutually exclusive scenarios.
% \textit{(i) For $(n - 1) \tau $ large enough (typically greater than 5)}, we approximate the binomial distribution by a normal distribution, so that the number of positive samples, with 95\% probability, is greater than $1 + (n-1)\tau - 1.64 \sqrt{(n-1)\tau(1-\tau)}$. We have previously seen that the distribution of the $C_t$ became favorable for $k>2$ positives, so we must have: $ 1 + (n-1)\tau - 1.64 \sqrt{(n-1)\tau(1-\tau)} > 2 $, which implies that $\tau > 2.2 \frac{1}{n} + o(\frac{1}{n})$. Thus as soon as the distribution of $\tau$ is above these values, then the sensitivity does not change.

% \textit{(i) For $(n - 1) \tau $ small}: in the regimes that we are considering, this means that  
% The impact of the stochasticity is of the form:
% \begin{equation*}
%     \begin{split}
%     \mathbb{E}_{H_a}[\sum_{i=1}^n Y_i]& =  \int (1-\pi)\pi (1 +  p(\tau) d\tau p(\pi) d\pi   \\
%     \end{split}
% \end{equation*}



 








==> COVID Pooled Testing Draft Paper 2/intro.tex <==
% !TEX root = main.tex

With an estimated 16\% of SARS-CoV-2 cases being asymptomatic and 50\% of detections occurring prior to symptom onset (\cite{he2020proportion,oran2020prevalence,pollock2020asymptomatic}), widespread surveillance testing plays a crucial role in monitoring and controlling the spread of SARS-CoV-2  (\cite{Larremore2020TestScreening.,gandhi2020asymptomatic,doi:10.1056/NEJMp2025631,dhillon2015ebola,nouvellet2015role,rannan2021increased}).  Yet in practice, the inherent logistical costs of widespread testing have severely limited its deployment at scale. Throughout the pandemic, testing needs have outstripped availability: in November 2020, the United States fell short of its COVID-19 testing objective by 48\%, performing a daily average of 1,193,000 tests out of the 2.3 million set as a minimum target (\cite{nyt}). Testing shortages continue to persist globally, as reported during the Spring 2021 surge in India (\cite{npr_india}) or as projected for the  "third wave" throughout Africa in Summer 2021  (\cite{bbc_africa}). 
%The need to vastly increase testing capacity has strained both the ability to respond to the COVID-19 pandemic, and 
The unprecedented surge in testing demand  has also strained the broader laboratory supply chain; from September 2020 through January 2021 in the U.S., shortages of testing materials (e.g. reagents, consumables, etc) significantly impacted day-to-day testing for both COVID-19 and other infectious diseases (\cite{asm_testing}). 
Consequently, despite rising vaccination rates in some parts of the world (at the time of writing), the threats of new variants, waning immunity, and localized outbreaks  
make the deployment of robust and continued large scale testing a priority.

In this context, pooled (or group) testing procedures have generated increasing interest during the pandemic (\cite{Abdalhamid2020AssessmentResources}). First proposed by \cite{Dorfman1943} to screen soldiers for syphilis, the simplest form of pooled testing is a two-stage hierarchical procedure in which multiple laboratory specimens are first combined and tested, and samples from positive pools are subsequently individually re-tested. Since then, pooled testing has been successfully employed in a number of applications,  ranging from the testing for low prevalence diseases (including HIV, chlamydia, and gonorrhea (\cite{McMahan2012InformativeScreening,wein1996pooled,tu1995informativeness,gaydos2005nucleic}), to the detection of genetically modified organisms in crops (\cite{yamamura2007estimation}).

Despite limited prior use of pooled testing for widespread epidemic management, the American Food and Drug Administration (FDA) approved its use for certain SARS-CoV-2 diagnostic tests in Summer 2020, with some restrictions. According to these guidelines, the sensitivity of the pooled procedure should be maintained above the threshold of 85\% (\cite{FDA2020CoronavirusTesting}). %In practice, the sensitivity and efficiency of the pooled sampling procedure is a function of the prevalence.
%FDA approval of pooled testing for SARS-CoV-2 was subject to the restriction that the the sensitivity (ability to detect positive samples) of pooled procedure must remain above the nominal threshold of 85\% . 
This desideratum must also be weighed against logistical feasibility of implementing pooled testing --- a tension recently described by the College of American Pathologists\footnote{\url{https://www.cap.org/covid-19/pooled-testing-guidance-from-cap-microbiology-committee}} and which can be summarized along the following two axes:\\
\indent \textbf{\textit{{(a) Logistics.}}} Prior to the pandemic, a substantial body of literature already considered better pooling designs ---  either by grouping specimens according to a set of covariates (\cite{McMahan2012InformativeScreening,chen2009group,bilder2010informative}), or by placing the samples into an array matrix (\cite{mcmahan2012two}) to allow the immediate identification of contaminated specimens without individual retesting. While these procedures can yield impressive efficiency gains from a purely statistical perspective, they simultaneously introduce more room for errors in specimen handling: if performed manually, specimen pooling can increase risk of specimen confusion and cross-contamination while increasing lab handling times. Automated robots become  essential for aliquoting and attributing samples to pools following complex optimal designs. Thus, while mathematically optimal, these solutions are often difficult to implement without state-of-the-art (and often expensive) equipment.  \\
\indent \textbf{\textit{{(b) Context-dependent efficiency and sensitivity.}}} The sensitivity and efficiency (number of tests per sample) of pooled testing are known to be functions of the pool size and disease prevalence. The latter determines the probability that a pool contains at least one positive individual, and therefore, that all individuals in the pool require re-testing (\cite{Gastwirth2000The2}): larger pool sizes in low prevalence regimes ensure that fewer tests have to be carried out. Concurrently, pooling dilutes the amount of viral genetic material present in positive samples, thereby potentially reducing the sensitivity of the procedure. Previous studies have investigated the sensitivity of pooled testing under different prevalence levels in order to develop coarse recommendations for selecting an appropriate pool size at a given prevalence level (\cite{Kim2007ComparisonError,McMahan2012InformativeScreening}). Such studies typically assume independently and identically distributed (i.i.d) samples when estimating the appropriate pool size. However, such i.i.d assumptions may not be reasonable for SARS-CoV-2 given widespread community transmission and specimen collection procedures that capture highly connected networks --- a phenomenon virtually unique to an epidemic scenario, and irrelevant to the low-prevalence-disease monitoring that pooled testing has historically been used for. 

In fact, in many SARS-CoV-2 collection scenarios, infections and positive specimens are clustered, such as when testing students in dorms, coworkers in an office,  individuals in households, or classrooms of children on a weekly basis (\cite{wapo_schools, Adam2020ClusteringKong,Zhang2020FamilialAsymptomatic}). Transmission rates in these networks may be much higher than in less connected networks (Table \ref{table:tau_dist} in Appendix \ref{sec:appendix_sim}). By way of illustration, household transmission rates are estimated to vary from 4\% to 55\% (\cite{Koh2020})--- highlighting  transmission rates within close communities greater than the overall prevalence by orders of magnitude, but with significant uncertainty and heterogeneity. This leads us to a first lesson that we draw from our analysis: \\
\xhdr{Lesson 1} \textit{ The unprecedented data collection and sampling processes observed during the pandemic have severely compromised the validity of classical statistical pipelines for the analysis of data --- thereby  leading to an inaccurate evaluation of pooled testing and  potentially suboptimal deployment of this method. Statistical modeling  is key to rapidly and efficiently re-adapting existing procedures to this novel setting, but its relevance is contingent on being able to bridge   the gap between statistics-based optimality --- which strives to make the greatest efficiency gains --- and field-based optimality -- which is informed by practical constraints and logistical considerations. } 

To adapt to this novel situation, several studies have begun investigating the impact of deviations from the i.i.d setting on the sensitivity and efficiency of pooled testing. To account for \textit{non-independence},  \cite{Rewley2020SpecimenStudy} simulated correlations between consecutive persons in a testing queue, assuming an additive increased chance of a positive test given the previous person in line was positive. The simulations suggested that as the likelihood of clustered infections increased, pooling efficiency also increased, even with rising prevalence. Other simulation studies have similarly concluded that the Dorfman two-stage procedure is optimal when testing is performed on clusters of correlated individuals  (\cite{Deckert2020SimulationTesting, Lin2020PositivelyCosts}). So far, many of these studies have necessarily relied on simulating simplified settings, with arbitrary parameterisations and distributions and ignoring variability across pools. Few simulation studies have attempted to capture deviations from the \textit{identically distributed} hypothesis, in part because there is minimal practical applicability for incorporating information on individual level covariates relevant to infection risk. 

\indent Taking an experimental data-driven approach, \cite{Barak2021} examined Dorfman-based pooled testing on over 130,000 SARS-CoV-2 samples. Pool size was adaptively chosen based on predicted prevalence levels in the community. They found that the rate of positives in pooled samples was best predicted by sorting samples into batches according to their source (such as by colleges, nursing homes or health care personnel) and also incorporating epidemiological information about the probability of infection in these different sources. Overall, they observed that pooled testing performance exceeded expectations both in terms of efficiency and sensitivity, which they attributed solely to the fact that there is a nonrandom distribution of positive samples in pools. Thus, real-world data supports the push to develop easily adaptable pooled testing strategies that exploit the non-i.i.d nature of samples.  Due to rapidly changing SARS-CoV-2 prevalence, laboratories require practical tools that allow them to adapt their procedures to the context and populations they treat.

% These deviations from standard hypotheses can shift the expected performance of the pooled testing procedure by modifying the inputs along two orthogonal dimensions: (a) the effective pool size is typically smaller than actual pool size, due to violations of the independence assumptions --- thereby "reducing" the dilution effect --- and, (b) the effective prevalence can differ from global prevalence due to violations of the ``identically distributed" hypothesis: healthcare workers are typically more at risk than remote workers, school-age children might as well be more likely to contract the disease as they interact with other school children, etc. 

\xhdr{{Objectives}} 
%In the context of COVID-19, the appropriate and optimal conditions for deployment of pooled testing for COVID-19 surveillance remain an open area of research \cite{centers2020interim}. 
%In this paper, we propose to highlight lessons learned from the applications of statistical modeling to the design of practical, efficient and high throughput group testing strategies.
% Our objective is two-fold. \textit{(a) We show how integrating practical constraints into statistical modeling is crucial and can yield  unexpectedly efficient solutions}. To this end, we provide a simple model that measures the efficiency of pooled testing under correlations, and uses the lessons from \cite{Barak2021} in practical pooled sampling to guide our approach.
%     Extending their observations, our simple mathematical model shows that pooled testing can be efficiently optimized
% through natural deviations from the i.i.d hypotheses in the specimen collection process, allowing gains in sensitivity and efficiency
% up to respectively 30\% and 90\% greater than in an i.i.d setting.  Our modeling of correlations is informed by real-data and practical constraints and, allows for the simultaneous consideration of non-independence and
% population heterogeneity; 
%      \textit{(b) We investigate and produce practical and actionable recommendations that are ready for deployment during the COVID-19 pandemic}. For this reason, we focus on the Dorfman two-stage procedure rather than more mathematically optimal, but unscalable, pooling procedures.\\
We have two primary objectives:
 \begin{enumerate}[nosep]
    \item \textit{Show how a simple pooling method and accounting for correlated specimens in statistical modeling can yield unexpectedly efficient solutions}. To this end, we provide a straight-forward model that measures the efficiency of pooled testing under correlations, as well as formalizes and extends the lessons from \cite{Barak2021} in practical pooled sampling. 
    \item \textit{Investigate and produce actionable recommendations that are ready for deployment during the COVID-19 pandemic}. For this reason, we focus on the Dorfman two-stage procedure rather than more mathematically optimal, but unscalable, pooling procedures. 
\end{enumerate} 
\indent We organize our discussion around three main lessons that our investigation of pooled testing for SARS-CoV-2 samples has taught us: (1) the importance of leveraging setting-specific information to optimize testing, (2) the necessity of evaluating efficiency through a set of several, practically meaningful measures, and (3) the importance of modeling the impact of uncertainty and/or heterogeneity. We show that pooled testing can efficiently identify infectious individuals despite natural deviations from i.i.d hypotheses in the specimen collection process, with little detrimental effect on the accuracy of the procedure; %(sensitivity, sensitivity relative to individual testing,  expected number of missed cases per sample).
Gains in sensitivity and efficiency can in fact be as much as 30\% and 90\% respectively compared to i.i.d settings.  In contrast to existing studies, our modeling of correlations (i) is focused on understanding pooled sampling's heightened sensitivity through its effect on the viral load of the sample (measured as the cycle threshold ($C_t$) value), (ii) is informed by real data and practical constraints and above all, (iii) allows for the simultaneous consideration of non-independence and population heterogeneity.
%we frame this problem as a distortion of the law of probability of the number of positive samples per pool --- thereby allowing us to compute a correction to existing abaci, the impact on the volatility of metrics of interest, and preserving the ease of its deployment. 
%We highlight the robustness of these results despite the uncertainty in input estimate (transmission rate and prevalence) using prior distributions on the parameters derived from real-world data.
%\item 

% To make our framework readily implementable and accessible, we present an RShiny interface that acts as an end-to-end pipeline for users looking to conduct group testing and select parameters relevant to their testing setting. Finally, throughout this paper, we strive to highlight lessons in data analysis that this pandemic has allowed to put forward.
%\end{enumerate}

% In particular, Wang, et al. (2020) estimated the effects of dilution on positive percent agreement (PPA) with individual testing and efficiency of a two-stage pooling strategy, accounting for prevalence, viral load distribution, and assay sensitivity [REF]. %They found that PPA was dependent on the proportion of positive tests, cycle threshold ($C_t$) distribution, and assay LoD, and was greater for smaller pool sizes. 
% The authors provide a series of grids and plots serving as an abacus and allowing users to read off the best pool size depending on the local prevalence. \\

==> COVID Pooled Testing Draft Paper 2/mathematical_framework.tex <==
% !TEX root = main.tex

This section focuses on a three-fold approach to understanding the impact of deviations from the i.i.d hypotheses on the $C_t$ value: (1) We introduce a model that accounts for positive correlations between samples; (2) We expand upon the observation by \cite{Barak2021} that pooled testing achieves improved sensitivity of pooled testing due to the "hitchhiker effect" --- a phenomenon whereby the detection of weakly positive tests is improved by borrowing strength from strongly positive tests --- by providing a mathematical framework to quantify this effect; and (3) We use this framework to show how positive correlations between samples can further improve the sensitivity of the pooling procedure.  
%Such a model is indeed key to find optimal deployment strategies for pooled testing and to quantify their benefits, and to support the empirical results of Bakar et al \cite{Barak2020LessonsTests} on the lack of severe detrimental effects of the pooling on sensitivity.

\subsection{A Network Model for Pooled Specimens}

%In this section, we propose a simple model to describe probability laws for the amount the amount of viral material per pool.

\xhdr{Modeling Non-independence (Network Effect)} Consider that there are $n$ samples in each pool. We assume that all the specimens are sampled from a network (co-workers, classroom, household, etc.) modeled by a fully connected graph on $n$ nodes with edges indicating potential transmission between a given node and its neighbors. We denote by $\tau$ the network transmission probability between individuals in the pool (that is, the probability that an infected member infects another subject in the network), so that each edge $e_{ij} = \tau$ represents the probability that node $i$, if infected, transmits the disease to node $j$; in epidemiology, this parameter is commonly referred to as the secondary attack rate (SAR).  The community transmission probability, or equivalently, the prevalence in the population, is denoted by $\pi$. Let us denote as $Y_i$ the indicator variable that specimen $i$ is infected ($Y_i = 1$ if individual $i$ infected, $0$ otherwise). Since transmission can occur within the network or in the community, we decompose $Y_i$ as follows: (1) Let $T_i^{(cmty)}$ be the random variable indicating infection of individual $i$ from outside the group (community transmission), and (2) Let $T_i^{(ntw)}$ indicate infection from within the group (network transmission). The existence of a network effect is captured by writing the infectious status of individual $i$ as the sum: 
$$  Y_i = T_i^{(\text{cmty})} + (1-T_i^{(\text{cmty})})T_i^{(\text{ntw})} \quad \text{with } T_i \in \{0,1\},\quad  T_i^{(\text{cmty})} \indep  T_i^{(\text{ntw})}  \hspace{1cm}(M_1),$$
so that $$ \mathbb{P}[Y_i=1] = \mathbb{P}[ \{T_i^{(\text{cmty})}=1\} \cup \{T_i^{(\text{net})}=1\}].$$ 

Network and community transmissions are themselves modeled as Bernoulli variables and tied to the SAR $\tau$ and prevalence $\pi$ through the relations: 
$$\mathbb{P}[T_1^{(\text{cmty})} = 1 ] =\pi  \hspace{1cm} \text{ and }  \hspace{1cm} \mathbb{P}[T_1^{(\text{ntw})} = 1 | Y_2, \cdots, Y_n] = 1 - (1-\tau)^{\sum_{i=2}^n T_i^{(\text{cmty})}}.$$ In other words, network transmission is modeled as independent Bernoulli($\tau$) variables across edges, so that the probability that this transmission route fails is the product of the probability of failure across each edges: $\mathbb{P}[T_1^{(\text{ntw})} = 0 | Y_2, \cdots, Y_n]  = (1-\tau)^{\sum_{i=2}^n T_i^{(\text{cmty})}}$.  A given pool can have a total of $K \le n$ positive samples, $k$ of which are infected from the community and $K-k$ of which are infected from within the network.\\

\begin{figure}[h]
    \centering
    \includegraphics[width=10cm]{Figures/net_effect.png}
    \caption{Representation of the network effect on the infectious status for any given node. This highlights the higher risk of sample $i$ testing positive as soon as another sample in the network is also positive.}
    \label{fig:net_effect}
\end{figure}


\xhdr{Modeling Non-identical Distributions (Heterogeneous Infection Probabilities)} Individuals within a network are exposed to various levels community transmission risk depending on a number of covariates, including age, profession, and lifestyle. This risk also varies considerably with time and epidemic kinetics (new variants, vaccination levels, etc.). At the granular level, this can be captured by introducing node covariates $X_i$'s and allowing heterogeneous community infection rates:
$$ \forall i, \qquad \mathbb{P}[T_i^{(\text{cmty})} = 1] = \pi  + f(X_i)  + \epsilon_i$$
where $\pi$ is the general community prevalence level, $f(X_i)$ reflects deviations from this baseline level depending on a set of covariates (e.g. profession, lifestyle), and $\epsilon_i$ is a noise term capturing the stochasticity of the prevalence (e.g. temporal effects) and/or potential subject effects. 
Several studies have investigated using subject-level covariates to inform the risk function $f$, by classifying individuals either as high/low risk (\cite{McMahan2012InformativeScreening,bilder2019informative, donnat2020bayesian}), or to inform retesting (\cite{bilder2012pooled}).
However, in the context of the COVID-19 pandemic, and due to the necessary volume and frequency of testing, introducing individual subject covariates yields impractical solutions: the collection of subject-level covariates and dispatching of samples in pools according to their risk slows down the procedure and yields intricate pooling designs which are not feasible at scale. As such, we  propose simply leveraging the specimen collection process to assume similar behaviors and covariates across pooled specimens ($f(X_i) \approx f(X_j) \quad  \forall i, j$) so that pools on any given day can be considered homogeneous, and that random effects --- due for instance to temporal variations, different variants, etc --- are at the pool (instead of the individual subject) level: 
$$ \forall i, \qquad \mathbb{P}[T_i^{(\text{cmty})} = 1]  = \pi  + \epsilon_{\text{pool}}.$$
%and where the estimate of the prevalence is a function of time and community (ie, graduate students, etc.).


\xhdr{Discussion} This simple model allows us to capture a variety of situations. In particular, (i) the value of the SAR $\tau$ drives the balance between community and network transmission: the higher the value of $\tau$, the more likely that any community transmission will yield more than one secondary infection in the pool. Conversely, for $\tau=0$, there is no network transmissions and the samples are independent.  (ii) Assuming this notation, the standard i.i.d case studied in the literature is a homogeneous, fixed effect model and assumes $f=0$ and $\epsilon=0$  (so that $\forall i, \quad \pi_i = \pi$) and $\tau=0$. We refer to the uncorrelated, i.i.d scenario with prevalence $\pi$ and pool size $n$ as our null model $H_0(\pi, n)$, and to the correlated, heterogeneous one as the alternative $H_a(\pi + f,  n, \tau)$. (iii) This model allows us to study the law of the number of infected samples in the pool. As we will describe in subsequent subsections, the shift in probability distribution leads to improved performance of the pooling procedure. In Table~\ref{tab:properties}, we summarize the properties of the distribution of number of positive samples per pool under both models. 

\begin{table}
    \caption{Comparison of the properties of the number of infected samples per pool (size=$n$), with, and without correlation. All the derivations are provided in Appendix \ref{sec:appendix_comp}. Note, in particular, the shift in the expected number of samples as a function of the network  transmission rate (or SAR), $\tau$.}
    \label{tab:properties}
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{{@{}lll@{}}} 
    \hline
       Quantity  & $H_0(\pi, n)$ &  $H_a(\pi,  n, \tau)$\\  
    \hline
       Distribution  & $\sum_{i=1}^n Y_i \sim \text{Binomial}( n, \pi ) $  &  $\sum_{i=1}^n Y_i$ + Binomial$(\sum_{i=1}^n Y_i, \tau )$ ;  with $\sum_{i=1}^n Y_i \sim \text{Binomial}( n, \pi ) $  \\ [10pt]
       
       $\mathbb{P}[Y_i=1]$  &  $\pi$  & $1-(1-\pi)(1-\pi\tau)^{n-1}$ \\ [10pt]
       
       Correlation $c(Y_i, Y_j)$  & 0 & $\frac{(1-\pi)^2\Big[(1-\pi + (1-\tau)^2 \pi  )^{n-2}-  (1-\pi\tau)^{2n-2}\Big]}{{(1-(1-\pi)(1-\pi\tau)^{n-1})((1-\pi)(1-\pi\tau)^{n-1})}}$\\ 
       & & $=(1+\frac{1-\tau}{1+(n-1)\tau})\tau + o(\tau)$ \\ [10pt]
       
       Average number of & $n\pi$  & $n\pi$ + $\sum_{k=1}^{n-1} {n \choose k} \pi^k (1-\pi)^{n-k} (1-  (1-\tau)^k) (n-k)$ \\
       positive samples per pool & & $= n\pi ( 1 + (n-1)\tau) + o(n\pi)$\\[10pt]
       
       Average number of & $\frac{n\pi}{1-(1-\pi)^n}$  & $1 + \sum_{k=1}^{n-1} {n \choose k} \frac{\pi^k (1-\pi)^{n-k}}{1-(1-\pi)^n} (1-  (1-\tau)^k) (n-k)$ \\
       positive samples  & $\approx 1$ & $\approx( 1 + (n-1)\tau)$ \\  
          per contaminated pool    & & \\ [10pt]
          
        $\mathbb{P}[\sum_{i=1}^n Y_i=0] $ & $(1-\pi)^{n}$ &  $(1-\pi)^{n}$  \\ [10pt]
        
        $\mathbb{P}[\sum_{i=1}^n Y_i=k], k>0$&  ${n \choose k} \pi^k (1-\pi)^{n-k}$ & $ \sum_{j=1}^k {n \choose j}  \pi^j (1-\pi)^{n-j} {n - j \choose k-j} (1-  (1-\tau)^j)^{k-j} (1-\tau)^{ j (n-k)}$ \\[.1cm] \hline 
    \end{tabular}}

\end{table}

Since (as in Table~\ref{tab:properties}), the probability of the number of positive samples per pool is a complex polynomial function of $\tau$, we propose an approximation when the prevalence is small. This allows us to gain greater insight into the intricate interplay between $\tau$ and $\pi$, without hindering the utility of the analysis since pooled sampling is predominantly deployed in low prevalence settings. More precisely, we make the following assumption:
\begin{quote}
\textbf{Assumption 1- Low Prevalence}: We assume that the prevalence is such that $\pi n \leq 0.10$. To put this number into context, this scenario is aligned with situations observed in Summer 2020 or Spring 2021 in Europe and the U.S.: in early June 2021 for instance, the reported prevalence of COVID-19 in the United Kingdom was estimated around 0.70\%, which would allow us to look at pool sizes of up to 15, or to sizes of up to 50 for low prevalence levels under 0.2\% observed in some parts of the world (such as for instance Israel \footnote{Data from \href{https://ourworldindata.org/covid-cases}{Our World in Data} (percentage of positive samples per test). For the sake of completeness, a chart is provided in Figure~\ref{fig:comp} in Appendix \ref{sec:appendix_complementary}.}) in late June 2021 . This is a convenient threshold that allow us to simplify the analysis while still providing insight into the interplay between community and network transmission, as highlighted by the two following observations.
\end{quote}

\noindent \textbf{Observation 1: } Under Assumption 1 ($\pi n \leq 0.10$), the probability that under $H_0$, there are two or more infected samples in the pool is less than $.01$.
This follows from the following simplification:
\begin{equation*}
    \begin{split}
        \mathbb{P}_{H_0}[\sum_{i=1}^n Y_i > 1] &= 1- (1-\pi)^{n} - n\pi(1-\pi)^{n-1} = 1 - (1-\pi)^{n-1} ( 1 + (n-1)\pi)\\
        &\leq  1 -  (1-(n-1)\pi + \frac{(n-1)(n-2)}{2}\pi^2 - \frac{(n-1)(n-2)(n-3)}{6}\pi^3 + o(n^3\pi^3) )  \\
        &\times( 1 + (n-1)\pi)\\
        &\leq \frac{n(n-1)}{2} \pi^2 -n \frac{(n-1)(n-2)}{3} \pi^3 +  o(n^3\pi^3)\\
        &\leq 0.005. 
    \end{split}
\end{equation*}
%and where the remainder $O(n^3\pi^3)$ is negative.
Similarly, in a pool with at least one infected sample, we can show that:
$$     \mathbb{P}[S \geq 2| S \geq 1 ] \leq  \frac{n}{2}\pi \leq 0.05.$$
(see Appendix \ref{sec:appendix_comp} Eq.\ref{eq:eq} for details). This means that with 95\% confidence, an infected pool contains only a single infected sample. This fact will be useful to simplify our computations in the subsequent paragraphs.

\noindent \textbf{Observation 2: }  Concurrently, in this scenario, the number of positive samples per pool \textbf{with correlation} is: 
%$\mathbb{E}_{H_a}[\sum_{i=1}^n Y_i] = n\pi + n\pi(1-\pi)^{n-1}\tau(n-1) + O(n^3\pi^3)= n\pi ( 1 + (n-1)\tau) + O(n^3\pi^3)$ and where the remainder is bounded by $n^4\pi^3< 0.005n$.
%Thus, the total mean number of people infected is 
$\mathbb{E}_{H_a}[\sum_{i=1}^n Y_i]= n\pi + n(1-\pi)  (1- (1-\tau\pi)^{n-1}) $ while the probability that there are more than 1 infected samples in the pool is:
\begin{equation*}
    \begin{split}
        \mathbb{P}_{H_a}[\sum_{i=1}^n Y_i > 1] &= 1- (1-\pi)^{n} - n\pi(1-\pi)^{n-1} (1-\tau)^{n-1}\\ 
        &= \mathbb{P}_{H_0}[\sum_{i=1}^n Y_i > 1]   + \big( 1- (1-\tau)^{n-1} \big) n\pi(1-\pi)^{n-1}  \\ 
        &\geq  \mathbb{P}_{H_0}[\sum_{i=1}^n Y_i > 1] \Big( 1 +  \frac{2(1-(1-\tau)^{n-1})}{(n-1)\pi}  - \frac{2((n+1)((1-\tau)^{n-1}  -1))}{3(n-1)} \Big)\\
        &\approx  200  (1 -(1-\tau)^{n-1}) \mathbb{P}_{H_0}[\sum_{i=1}^n Y_i > 1] \quad \text{ under Assumption 1.}\ 
    \end{split}
\end{equation*}
where the last line follows from the fact that the dominating term is in $\frac{1}{\pi} \geq 100$, whereas the others  are of order $\sim 1$ (see Appendix \ref{sec:appendix_comp}  Eq.~\ref{eq:proba_ha} for details).  This illustrates the striking difference in behavior between the distribution of positive samples with and without correlation: the probability of having more than two samples in a correlated pool increases rapidly, as the inverse of the prevalence. 
%As a direct consequence, the mean increases by $k$ new infections compared to the null as soon as $\tau \geq \frac{1}{\pi}( 1 - (1-\frac{k}{N(1-\pi)})^{1/(N-1)} \approx  \frac{k}{N(N-1)(1-\pi)\pi} + o(1)$.


\noindent \textbf{Observation 3: } Conditional on the pool being positive, the expectation of number of positive samples per pool \textbf{with correlation} can be well approximated by: $\mathbb{E}_{H_a}[\sum_{i=1}^n Y_i] = 1+(n-1) \tau +  \frac{1}{2}(n-1)(1-\tau)((n-2) \tau +1) \pi + O(n^3\pi^3)$, where the remainder is bounded by $n\pi$ (proof in Appendix \ref{sec:appendix_comp})) --- thereby shifting the mode of the number of infected samples (conditional on  $\sum_{i=1}^n Y_i>1$) from 1 under $H_0$ (with 95\% confidence) to $ 1 + (n-1)\tau + 0.05 (n-2)(1-\tau)\tau \approx 1 + (n-1)\tau  $ with correlations. The number of positive samples in infected pools thus increases roughly linearly with the SAR. This further supports the observation by \cite{Barak2021} regarding the existence of positive correlations between samples: our relationship quantifies the effect and the strength of the interactions on the distribution of the number of positive samples per pool. This relationship is illustrated in  Figure \ref{fig:increments_tau}, where we show the minimum value of $\tau$ required to induce an increment of $k=1, \cdots, n-1$. We observe that very low values of $\tau$ can shift the distribution quite considerably: for a pool size of 70, in low prevalence regimes, a value of $\tau=0.001$ is sufficient to increase the expected number of samples in positive pools by 2. In short, in an i.i.d setting, the probability of observing strictly more than one sample is extremely low. Our simple model highlights the fact that with moderate correlations between samples, observing more than one sample becomes in fact highly probable --- whereas it is unlikely with high probability (0.95) under the i.i.d null.

%$\log_2(n)/28 + 1$. The latter stems from the observation made in the previous paragraph that:
% $$C_{t}  \overset{D}{=} \log_2(\sum_{S} 2^{-C_t^{i}}) -\log_2(n) \geq  - \sum_{S} C_t^{i} + log_2(n) $$
% where the previous inequality follows by concavity of the log. Thus, in average, to beat the performance of individual sampling we must have: $-k \mathbb{E}[C_t^{i}] + \log_2(n) \leq  - \mathbb{E}[C_t^{i}]$, and thus $k \geq \frac{\log_2(n) }{\mathbb{E}[C_t^{i}]} + 1$, with $\mathbb{E}[C_t^{i}] \approx 28$


\subsection{Modeling the Hitchhiker Effect}

Armed with the previous set of observations, we now turn to the quantification of the "hitchhiker effect" observed by \cite{Barak2021}--- a phenomenon whereby the detection of weakly positive samples borrows strength from strongly positive samples in the pool, thus increasing their chances of detection. This requires us to model the influence of the number of contaminated samples in the pool on the viral load present in the sample, as detailed in the generative model presented in Figure~\ref{fig:graph_model}.  This viral load is measured during testing by the \textit{cycle threshold} ($C_t$) of the pooled sample. The $C_t$ in reverse transcription polymerase chain reaction (RT-PCR) refers to the number of cycles needed to amplify viral RNA to reach a fixed background level $T$ of fluorescence at which the diagnostic result of the real-time PCR changes from negative (not detectable) to positive (detectable)\ (\cite{tom2020interpret}). Since at every cycle, the amount of viral RNA is (roughly) doubled, the $C_t$ value is thus an indirect measure of the viral load $n^{(0)}$ in the sample:

\begin{equation}
T = n^{(0)} 2^{C_t}  \implies C_t = \log_2(T/n^{(0)})
\label{eq:ct} 
\end{equation} 

The amount of viral material determines the sensitivity of the test: according to the previous equation, the higher the amount of viral material, the lower the $\text{C}_t$ value and the higher the probability of detection (Figure~\ref{fig:sens}).

\begin{figure}[ht]
    \includegraphics[width=\textwidth]{Figures/schema2.png}
    \caption{Graphical model for the procedure: the probability of a positive pooled test is a function of the number of infected samples (through community  and network  transmission) through the pooled $C_t$ value.}
    \label{fig:graph_model}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/increments_tau2.png}
    \caption{Minimum value of $\tau$ required to shift the expected number of infected samples in a pool by $k$ as a function of the pool size and the overall community prevalence $\pi$. NA values are highlighted in grey. We note that small values of $\tau$ (e.g, 0.01, here represented by the yellow color) can already yield an increase of 1 or more in the expected number of positive samples.}
    \label{fig:increments_tau}
\end{figure}


\begin{figure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \centering
    \includegraphics[width=\textwidth, height=4cm]{Figures/lod3.pdf}
    \caption{Pool size vs LOD and percentage of individual samples above the LOD}
    \label{fig:lod}
     \end{subfigure}  
     \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth, height=4cm]{Figures/sensitivity_ct.png}
    \caption{Sensitivity of the test as a function of the $C_t$ value}
    \label{fig:sens}
 \end{subfigure} 
     \caption{Probabilistic model for the metrics of interest and sensitivity as a function of the $C_t$ value}
\end{figure}

\xhdr{Effect of Dilution on $\text{C}_t$ Values}  Since by Eq. \ref{eq:ct}, $\text{C}_t = \log_2(T/n^{(0)})$, lowering the initial amount of viral material in the sample $n^{(0)}$ increases the $\text{C}_t$ value --- thus potentially lowering the initial viral load below the limit of detection and decreasing the sensitivity of the test. In fact, denoting as $\text{C}_{t}^{(i)}$ (respectively $n_i^{(0)}$) the individual samples' $\text{C}_t$ values (respectively  initial viral load), we can write the $\text{C}_t$ value for the dilution as:

\begin{equation} 
\begin{split}
    C^{\text{dilution}}_t &= \log_2(T) - \log_2(\frac{\sum_{i=1}^n n_{i}^{(0)}}{n})= \log_2(T) - \log_2(\frac{\sum_{i=1}^n T Y_i 2^{-C_{t}^{(i)}}}{n})\\
     &= - \log_2 ({\sum_{i=1}^n  Y_i2^{-C_{t}^{(i)}}}) +\log_2(n) 
    \end{split}
    \label{eq:dilution_ct}
\end{equation} 
 
Consequently, as shown in Eq. \ref{eq:dilution_ct},  the sensitivity of the pooled test is a function (through the $\text{C}_t$ value) of the number of positive tests per sample. Note that while the samples' infection status $Y$ are correlated, given the $Y_i$'s, the $\text{C}_t$ values can themselves be considered as independent --- that is, there is no evidence (at least, at the time of writing) of the value of the $\text{C}_t$ depending on context (e.g. a sample's corresponding age, gender, genetics, or virus strain). To study the efficiency of this procedure, we consider the  following  two sufficient and mutually exclusive scenarios:
 
 \begin{itemize}
  \setlength\itemsep{1em}
     \item \underline{For $\sum_{i=1}^n Y_i=1$ infected sample in the pool} (which, without loss of generality, we assume to be the first sample), the $\text{C}_t$ of the dilution is distributed as $ C^{\text{dilution}}_t  \overset{D}{=} C^{(1)}_t + \log_2(n)  $: i.e. the dilution translates the distribution of the $\text{C}_t$ value by $\log_2(n)$, and the impact on the sensitivity can be computed directly by translating the sensitivity curve by  $\log_2(n)$. As highlighted by \cite{Barak2021}, for a limit of detection for an individual $\text{C}_t$ value of 40, this means that pooled samples with only one positive sample could only be detected for samples under a $\text{C}_t$ value of $40 - \log_2(n)$; for example, with $n=8$, this would mean a limit of detection corresponding to a $\text{C}_t$ of 37, or for a pool size of $n=20$, a $\text{C}_t$ of 35. It is thus important to assess the stringency of these thresholds in the population being tested. To illustrate this, Figure \ref{fig:lod} provides a visualization of the evolution of the limit of detection and proportion of samples above the limit of detection in a real data set, corresponding to $\text{C}_t$ from positive samples from a Stanford hospital (see Appendix \ref{sec:appendix_sim}). In this case, the proportion of positive samples above the limit of detection $40 - \log_2(n)$ stays below 15\% (thus yielding a sensitivity around the CDC guideline of 85\%, since the sensitivity of the PCR is above 99\% for $C_t <34$) for pool sizes up to size 30. As such, in this particular population, the dilution effect is not overly detrimental to the accuracy of the test.  \cite{Barak2021} further argue that, due to  dwindling infectiousness as $\text{C}_t$ values increase, falsely negative samples with $\text{C}_t$ values 37 and above are less consequential than samples with lower $\text{C}_t$ --- thus mitigating the impact of the dilution on the efficiency of the testing procedure.
     
     \item \underline{For $\sum_{i=1}^n Y_i = k \geq 2$:}  Assuming without loss of generality that the $k$ first samples are positive, we have, by Taylor expansion around the minimum $\text{C}_t$:
     $$C^{\text{dilution}}_t  \overset{D}{\approx} \min_{j \in [1,k]}{C_t^{(j)}} + \log_2(n)  + \frac{1}{\log(2)} \sum_{i\neq \text{argmin}C_t^{(j)} }   2^{ \min_{j \in [1,k]}{C_t^{(j)}} -C_{t}^{(i)}}.$$
     (See Appendix \ref{sec:appendix_comp} for details.) Since the distribution of the $\text{C}_t$ values is heavily skewed, $2^{ \min_{j \in [1,k]}{C_t^{(j)}} -C_{t}^{(i)}} << 1$ with high probability so that $C^{\text{dilution}}_t  \overset{D}{=} \min_{j \in [1,k]}{C_t^{(j)}} + \log_2(n)$  with a good approximation. We provide a visualization of the distribution of the minimum $\text{C}_t$ over a random sample of $k$ $\text{C}_t$ values in our example population in Figure \ref{fig:min_ct}. While this figure uses data from a specific population, we expect this phenomenon to generalize across other populations, since $\text{C}_t$ values are known to exhibit important spread (\cite{Tso2021}). 
     (see Appendix \ref{sec:appendix_comp}). This fact is simply a formalization of the observations by \cite{Barak2021} that the $\text{C}_t$ value of the pooled sample is dominated by the value of the minimum. Thus, for a weakly positive sample (high $\text{C}_t$) to be detected, it is sufficient for it to be combined with a strongly positive sample. We further add to this argument that as the number of positive samples $k$ in the pool increases,  we expect the distribution of the dilution to be increasingly small (and eventually counterbalance the  $\log_2(n)$ offset).  %This extends the "hitchhiker" effect discussed in  \cite{Barak2021}  --- a phenomenon whereby weakly positive samples are combined with strongly positive samples, which increases their chances of detection. 
     To quantify the hitchhiker effect under correlation, we use Monte Carlo simulations to model the behavior of the dilution's $\text{C}_t$. We display the results in Figure \ref{fig:dilution}, where we show the distribution of the $\text{C}_t$ values in our reference population in various dilution effects, and different number of positive samples per pool. Note that for as few as $k=2$ samples, the distribution of the $\text{C}_t$ is comparable to the distribution of individual $\text{C}_t$, and, for these pool sizes, having three positive samples in the pool yields a $\text{C}_t$ distribution for the dilution with a smaller mode. 
 \end{itemize}
 
 The added benefit of this simple formalization is to allow us to study the hitchhiker effect when the independence assumption is violated. Let us consider the low prevalence setting of Assumption 1 ($\pi n <0.10$), and summarize these results as follows.\\
 
 \noindent \textbf{Observation 4.}\\
\textbf{ \underline{(a) i.i.d Case}} For a pool size $n$, by the total law of probability formula, the $\text{C}_t$ value of the dilution is a mixture of n distributions: 
       $$C_t \overset{D}{\approx} -\log_2(n) +  \sum_{k=1}^n 1_{\sum_{i=1}^n Y_i = k}  \min_{1\leq j \leq k} {C_t^{(i)}}$$
       Since in this setting, given that the pool is positive, the probability of having more than two samples is below 0.01, we have:
       $$C_t \overset{D}{\approx} -\log_2(n) +  C_t^{(1)}$$ so that the $\text{C}_t$ value behaves like a translated curve.\\
      \textbf{ \underline{(b) Network effects}} Assuming positive correlations between samples, by Observation 3, we know that we expect $(n-1)\tau$ more samples than under the null hypothesis. This means that the distribution of the minimum $\text{C}_t$ is more heavily skewed towards strongly positive samples, thus ensuring a better probability of detection in the pool.  In fact, we show in Appendix \ref{sec:appendix_comp} Eq.\ref{eq:ct} that the probability that a pooled $\text{C}_t$ with $K$ positive samples exceeds the average individual $\text{C}_t$ value is given by:
      $$  \mathbb{P} [ \min_{i \leq K} (C_{t}^{(i)}) + \log_2(n) > \mathbb{E}[C_t^{(i)} ]   ]  \leq  0.52^{K}  (1 + 0.11 K \log_2(n))  $$
 Thus the probability that the $\text{C}_t$ value of the mixture is greater than the expected $\text{C}_t$ of the individual samples is less than 0.67 for $K=2$, and 0.45 for $K=3$ (assuming worse case $n=100$). Thus, after $K=2$ to $3$ positive samples, the hitchhiker effect ensures that the $\text{C}_t$ value of the mixture will be favorable. While this result uses data from our reference study, we expect the behaviour exhibited here to generalize across populations.
      
      
To summarize, in this section, we have shown through simple derivations, backed by simulations, that the dilution only induces  a significant drop in sensitivity if a single sample is positive, but that this effect shrinks as the number of positive samples in the pool increases --- thus confirming and quantifying empirical observations made by \cite{Barak2021}. This allows us to conclude:\\
\xhdr{Lesson 2} \textit{Simple models tailored to the relevant statistical assumptions are useful. The realization that correlated/clustered specimen sampling could yield such considerable gains in $\text{C}_t$ value is only possible through a careful consideration of practical field constraints and observed measurements.}
     
\begin{figure}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \centering
    \includegraphics[width=\textwidth, height=5cm]{Figures/ct_dilution.pdf}
    \caption{Distribution of the minimum $C_t$}
    \label{fig:min_ct}
     \end{subfigure}  
     \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth, height=5cm]{Figures/Density.pdf}
    \caption{Ct value of the dilution}
    \label{fig:dilution}
 \end{subfigure} 
     \caption{Effect of the dilution on the $C_t$ value}
\end{figure}

      %In  
%Since this distribution is difficult to manipulate, we look at the impact of the SAR $\tau$ on a set of characteristics of the distribution: the mean and standard deviation.  


% \xhdr{Assumption 1} In real-life scenarios, we do not expect many samples to be positives. 
% \xhdr{Assumption 2} The network-effect changes the distribution  of the number of positive samples 


% This directly follows from the following recursion formula:  
% \begin{equation}
%     \begin{split}
%          C_{t, k+1}^{\text{dilution}} & \overset{D}{=}  C_{t, k}^{\text{dilution}}  - \log_2 \left( 1+  \frac{2^{-C_{k+1}}}{\sum_{i=1}^k  2^{-C_i}} \right) \\
%          &= C_{t, k}^{\text{dilution}}  - \log_2 \left( 1+  \frac{2^{-C_{k+1}}}{n 2^{-C_{t, k}^{\text{dilution}}}} \right) \\
%          \implies  C_{t, k+1}^{\text{dilution}}  \approx & \begin{cases}
%          C_{t, k}^{\text{dilution}}  - C_{t, k}^{\text{dilution}} + C_{k+1} - \log_2(n) \quad \text{if } C_{t, k}^{\text{dilution}} >> C_{k+1}\\
%           C_{t, k}^{\text{dilution}}   +  \frac{2^{C_{t, k}^{\text{dilution}}-C_{k+1}}}{n }  
%           \quad \text{if } C_{t, k}^{\text{dilution}} < C_{k+1}\\
%          \end{cases}
%      %  C_{t, k+1}^{\text{dilution}} & \overset{D}{=}  C_{t, 1}^{\text{dilution}}  - \sum_{i=1}^k \log_2 ( 1+  \frac{2^{-C_{j}}}{n 2^{-C_{t, j}^{\text{dilution}}}} )  =  C_{t}^{\text{individual}}  + \log_2(n)  - \sum_{i=1}^k \log_2 ( 1+  \frac{2^{-C_{j}}}{n 2^{-C_{t, j}^{\text{dilution}}}} )
%     \end{split}
% \end{equation} \label{eq:ct_dilution_change}
% As shown above, the most significant decrease in sensitivity occurs with only a single positive in the pool. For a large number of positive samples, the dilution has a positive effect and lowers the Ct value --- thus ensuring better sensitivity. Thus, as the number of positive samples increases, $C_{t, k+1}^{\text{dilution}} \approx C_{t, k}^{\text{dilution}}  - \frac{1}{\log(2)}\frac{2^{C_{t, k}^{\text{dilution}}-C_{k+1}}}{n } $

% The previous expression yields the following observations:
% \begin{itemize}
%     \item The greater the difference between $C_{t, k}^{\text{dilution}}$ and $C_{k+1}$, the greater the amplitude between $C_{t, k}^{\text{dilution}}$ and $C_{t, k+1}^{\text{dilution}}$
% \end{itemize}




% \xhdr{Distribution Shift: Positives per Pool}  To understand the effect of the correlations on the sensitivity and the effective sample size, let us consider their effect on the law of probability for the number of positive samples per case. 

% \underline{$H_0$: Under the Null}: $S = \sum_{i=1}^n T_i^{\text{(community)}} \sim \text{Binom}(n, \pi) $, and the mean number of infected people is thus $n\pi$. Note that in the regimes that we are considering in this paper, $ n\pi \leq 1$, so that the mode of the distribution is in fact $0$, while the standard deviation is $\sigma_0 = n\pi(1-\pi)$.


% \underline{$H_a$: With the effect of correlations}:  $S = \sum_{i=1}^n T_i^{\text{(community)}} + \tilde{S} $ where $\tilde{S}$ denotes the sum of all network transmissions. 
% $\tilde{S}| S \sim \text{Binom}(N-S, 1-(1-\tau)^S)$
% Thus, the total mean number of people infected is $\mathbb{E}[S] = N\pi + N(1-\pi)  (1- (1-\tau\pi)^{N-1}) $ (see Appendix \ref{sec:appendix_comp} for the derivation).  As a direct consequence, the mean increases by $k$ new infections compared to the null as soon as $\tau \geq \frac{1}{\pi}( 1 - (1-\frac{k}{N(1-\pi)})^{1/(N-1)} \approx  \frac{k}{N(N-1)(1-\pi)\pi} + o(1)$.
% Figure~\ref{fig:increments_tau} shows a plot of the behavior of this quantity as a function of $\pi$ and k.






% \xhdr{The variance} One of the mains issues  of the pooled testing approach is that it runs the risk of introducing more variance in the results: the dilution of the samples has the potential to drive the  

% $$\mathbb{V}ar[m] = \mathbb{V}ar[\mathbb{E}[m|\sum_{i=1}^nY_i]] + \mathbb{E}[\mathbb{V}ar[m|\sum_{i=1}^nY_i]]   $$

% In this case, we can show that the correlations in fact decrease the variance, since the effective number of samples is less that the observed one (to check):
% \begin{equation*}
%     \begin{split}
%         \mathbb{V}ar[m] &= \sum_{k=1}^K m_k^2\mathbb{V}ar[p_k] + \sum_{k=1}^K s^2_k p_k \\ 
%     \end{split}
% \end{equation*}








%





==> COVID Pooled Testing Draft Paper 2/metrics.tex <==
% !TEX root = main.tex



\subsection{Metrics of Interest and Benchmarks} 

Having studied the impact of the network transmission on the amount of viral material present in the sample, we now assess the impact of these departures from the traditional framework on our metrics of interest. To measure the efficiency of pooled testing under correlations, we introduce a set of four performance metrics, consistent with the group testing literature: the sensitivity ($s$), relative sensitivity ($s_r$) (which compares individual to pooled testing procedures), expected number of tests per sample ($\eta$), and proportion of missed cases per sample. 
%,and  number of missed positive cases per sample.

\xhdr{Sensitivity ($s$) and Relative Sensitivity ($s_r$)} Sensitivity ($s$) is the proportion of true-positives that are detected by the test, that is, the probability of a positive test result given that there is at least one positive sample in the pool. 

\begin{equation*}
    \begin{split}
        \textbf{Sensitivity: } s &= \mathbb{P}[\text{test is positive} | \sum_{i=1}^n Y_i \ge 1]\\
        &= \frac{\sum_{k=1}^n \mathbb{P}[\text{test is positive} \bigcap \{ \sum_{i=1}^n Y_i=k\}] }{\mathbb{P}[\sum_{i=1}^n Y_i \ge 1]} \\
        &= \frac{\sum_{k=1}^n \mathbb{P}[\text{test is positive} | \sum_{i=1}^n Y_i=k] p_k}{\mathbb{P}[\sum_{i=1}^n Y_i \ge 1]},
    \end{split}
\end{equation*}
with $p_k = \mathbb{P}[\sum_{i=1}^n Y_i = k]$. We assume that specificity (probability of a false positive) is zero.

However, tests are inherently imperfect, and such sensitivity might not be realistically achievable. As such, a more informative metric is the sensitivity of the pooled procedure, compared to individual testing (which we consider to be our ``gold-standard''). Relative sensitivity serves as a comparison of the probability of a positive test result in a pooled testing scenario to an individual testing scenario which might differ as a product of the dilution effect. 
\begin{equation*}
    \begin{split}
        \textbf{Relative Sensitivity: } s_r 
        &= \frac{\mathbb{P}[\text{test is positive} | \sum_{i=1}^n Y_i \ge 1]}{\mathbb{P}[\text{Individual test is positive} |Y_1  = 1]}\\
    \end{split}
\end{equation*}
Contrary to the sensitivity, this measure can take values in $\mathbb{R}^+:$ a relative sensitivity lower than one indicates a lower sensitivity of the pooled procedure relative to individual testing, whereas a value of $s_r$ greater than one would indicate a better sensitivity in the case of pooled testing with respect to individual testing.

Both sensitivities can be decomposed as a function of number of positive samples per pool and $\text{C}_t$ value as follows:
\begin{equation*}
    \begin{split}
    \forall x, \quad  \mathbb{P}[s > x]  &=  \int \mathbb{P}[s > x | C_t] p(C_t) dCt =   \int \sum_{k=1}^{n} \mathbb{P}[s > x | C_t] p(C_t, \sum_{i=1}^n Y_i = k) dCt \\
  &=   \sum_{k=1}^{n}  \mathbb{P}[ \sum_{i=1}^n Y_i = k]  \underbrace{\int \mathbb{P}[s > x | C_t] p(C_t|  \sum_{i=1}^n Y_i = k) dCt}_{=s_k, \text{ by definition}} \\
   &=   \sum_{k=1}^{n}  p_k   s_k \\
    \end{split}
\end{equation*}
where we have considered here the sensitivity of the test $s_k$ to be a function of the number of positives (marginalized over $C_t$ values). In light of our discussion of the effect of the network effects on the $\text{C}_t$ value of the dilution, we conclude that the existence of correlations has a positive effect on the sensitivities.


\xhdr{Expected Number of Tests per Sample ($\eta$)} This measures the efficiency of the pooled testing procedure. Since in the two-step Dorfman procedure every sample has to be re-tested if the pool is tested positive, the efficiency is:
\begin{equation*}
    \begin{split}
    \eta &=  \frac{1}{n} \times \mathbb{E}[1 + n \times \mathbb{P}[\text{test is positive}]  ] = \frac{1}{n} + \mathbb{P}[\text{test is positive}]\\
    &= \frac{1}{n} + \sum_{k=1}^n \mathbb{P}[\text{test is positive} |\sum_i Y_i =k] p_k
    \end{split}
\end{equation*}
This measure has to be compared against the benchmark value of $\eta_0 = 1$, which is the efficiency of the individual testing procedure (pool size $n=1$). However, it is important to note that the expected number of tests per sample must be considered in conjunction with other metrics, as it is only a partial indicator of the validity of the procedure. Indeed, a faulty test which is always negative will achieve the best efficacy $\eta=\frac{1}{n}$, but with zero sensitivity. %As such, in the spirit of the AUC and ROC curves used in Machine Learning, we consider the Area Under the curve defined by the plot of the effective number of tests vs sensitivity as the pool size varies as a way of comparing procedures.


 \xhdr{Proportion of Missed Cases per Sample} We also consider the proportion of cases that the grouped testing procedure fails to detect per test.
 $$=   \frac{\sum_{k=1}^n  k \mathbb{P}[\text{test is positive} | \sum_{i=1}^n Y_i=k] (1-p_k)}{\frac{1}{n} + \mathbb{P}[\text{test is positive}]}$$


\xhdr{Simulations} To illustrate our analysis, we perform Monte Carlo simulations and calculate our metrics of interest at varying pool sizes and values of $\pi$ and $\tau$.  We simulate two-stage pooled testing setting where individuals' infection statuses (positive vs. negative) are correlated, and compare this to our null model of assuming uncorrelated individuals. To make our analysis more realistic, the values of $\pi$ and $\tau$ are informed by fitting Beta distributions to published literature and data. For $\tau$, we fit Beta distributions to SAR values reported for a range of settings, including households with symptomatic index cases, households with asymptomatic index cases, transmission between spouses, healthcare settings, and from a child index case. For $\pi$, we fit Beta distributions to prevalence data at differing times over the course of the pandemic and geographic locations in the United States. The chosen time points and geographic locations are intended to be representative of varying prevalence levels and stages of the pandemic (e.g. rising cases, falling cases, etc). Details of the methodology for fitting the distributions, as well as information on the settings and distribution parameters are described in Appendix \ref{sec:appendix_sim}. Pool sizes range from $n$ of 1 to $n$ of 30.\\
\indent  To compute the sensitivity of the PCR test given a pool of size $n$ containing $1,...,n$ positive samples, we use empirically collected data on the distribution of $\text{C}_t$ values from \cite{Wang2021}, which is best represented by a Weibull distribution with shape parameter $s=4.5$ and scale $\eta = 30$. The distribution of the $\text{C}_t$ values depends on a number of factors, including the population tested (ie., hospital admissions vs general population, COVID variant, etc). To create a realistic distribution of $\text{C}_t$ values with the appropriate amount of spread, we sample and shift the Weibull distribution of \citeauthor{Wang2021}: we sample from their fitted distribution to create a mock distribution of individual $\text{C}_t$ values, and shift it to model a population in which 30\% of samples are above $\text{C}_t= 35$. \\
%This shift is done to account for the fact that the original data were collected during a time period when primarily symptomatic testing was done; when applied to widespread community testing, we would expect a higher proportion of the samples to have $C_t$ values greater than the LoD. 
%Results are presented for 30.0\% of $C_t$ values above the 95\% assay LoD, and for other proportions results are in the appendix.
\indent For each combination of $\pi$, $\tau$, and pool size, we calculate the metrics of interest (sensitivity, relative sensitivity, expected number of tests per sample, missed cases per sample), weighted by the probability of observing $k$ positives in that particular pool. We simulate the situation of testing a population of correlated individuals, where we either ignore correlation and erroneously treat the individuals as independent ($H_0$), or correctly consider networks of correlated individuals ($H_a$). In the null model, we make i.i.d assumptions and the expected number of positives per pool has a binomial distribution (probability of observing $K$ positives in $n$ trials (pool size) with success probability $\pi$ and $\tau = 0$. For the alternative model $H_a$, the probability of $K$ positives is computed exactly using the Poisson Binomial distribution (Appendix \ref{sec:appendix_sim}). 
%The KL divergence between the probabilities specified under the three alternative models and the null model is shown in Appendix Figure \ref{fig:kl_div_all}.

 \begin{figure}
    \includegraphics[width=\linewidth]{Figures/combined_fixed_plots.png}\hfill
  \caption{\textbf{Fixed Model}: Model-estimated parameters (sensitivity, relative sensitivity, expected tests per sample, missed cases per sample) by pool size, prevalence ($\pi$), and network transmission probability ($\tau$). Null (no correlation) model, individual testing, and FDA sensitivity threshold are also indicated, where relevant.}
   \label{fig:allmetrics_fixed}
\end{figure}


\xhdr{Discussion of Simulation Results}  Across all prevalence settings and levels of network transmission, the model that accounts for network transmission (correlations in pools) performs better in terms of higher sensitivity and fewer missed cases per sample than the null model (which ignores correlations) (Figure ~\ref{fig:allmetrics_fixed}). Accounting for correlations between individuals can result in large percentage increases in sensitivity over the null model; for example, for spousal network transmission in both low prevalence (e.g. Maine October 2020) and high prevalence (e.g. Alabama January 2021) settings, we observe 31.25\% and 19.14\% increases in sensitivity, respectively, compared to the null model (Table~\ref{table:summary_performance_fixed}). 

Comparing the sensitivity of the pooled procedure to individual testing, high levels of network transmission (such as observed between spouses and in a household with a symptomatic index case) results in sensitivity greater than the individual test, and far exceeding the minimum FDA threshold (0.85). In low prevalence settings or weak network transmission (such as healthcare settings or households with an asymptomatic index case), the sensitivity of the pooled testing procedure may fall below the FDA threshold (0.85) at large pool sizes. At sufficiently high prevalence levels (such as observed in Alabama in January 2021), pools of all sizes (including as large as 30) exceed the FDA threshold for pooled testing sensitivity. 

The pooled procedure also results in large decreases in the number of tests needed per sample, when compared to individual testing. Implementing pooled testing in Maine during October 2020 (low prevalence) among households with asymptomatic index cases, households with symptomatic index cases, and spouses could reduce the number of tests per sample by over 92\% in all three network transmission settings (Table ~\ref{table:summary_performance_fixed}). In higher prevalence settings, reductions in testing associated with pooled testing are more modest, but still upwards of 20\% (Table ~\ref{table:summary_performance_fixed}). 

From these results, we draw the following conclusion:\\
\xhdr{Lesson 3} \textit{The utility of pooled testing is context dependent, but statistical models informed by observed data in a range of prevalence and network settings demonstrate that accounting for non-i.i.d settings uniformly improves the expected performance of the procedure.}

\begin{table}
\caption{Expected performance of pooled testing for the fixed model under select prevalence, network transmission, and pool size scenarios.}
\label{table:summary_performance_fixed}
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1}
%\begin{adjustbox}{width=1.2\textwidth,center}
\resizebox{\textwidth}{!}{\begin{tabular}{@{}ccccc@{}} 
\hline
\multicolumn{3}{p{3.5cm}}{ }&
\multicolumn{2}{p{14cm}}{\centering \textbf{Fixed Model}}\\
 \cline{4-5}
 &   Network Transmission ($\tau$) & Prevalence ($\pi$)& 
 \multicolumn{1}{p{7cm}}{\centering \% Increase Sensitivity \\ Relative to $H_0$}&
\multicolumn{1}{p{7cm}}{\centering \% Decrease Tests/Sample \\ Relative to Individual Testing}\\
 \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{Pool Size n = 5}} 
& \multirow{2}{*}{Household Asympt. (0.012)}  
& Maine Oct. 2020 (0.2\%) &  0.62 &  79.35\\
& & Alabama Jan. 2021 (5.4\%) & 0.57 &  58.92\\[10pt]

& \multirow{2}{*}{Household Symptomatic (0.18)}  
&  Maine Oct. 2020 (0.2\%)  & 7.77 &  79.31\\
& &  Alabama Jan. 2021 (5.4\%) & 7.11 & 57.54\\[10pt]

& \multirow{2}{*}{Spouses (0.38)} 
&  Maine Oct. 2020 (0.2\%) & 13.02 & 79.28\\
& &  Alabama Jan. 2021 (5.4\%) & 11.85 & 56.55\\
 \hline
 
 \multirow{6}{*}{\rotatebox[origin=c]{90}{Pool Size n = 20}}
& \multirow{2}{*}{Household Asympt. (0.012)}  
& Maine Oct. 2020 (0.2\%) & 4.46 &  92.63\\
& & Alabama Jan. 2021 (5.4\%) & 3.12 &  36.88\\[10pt]
 
& \multirow{2}{*}{Household Symptomatic (0.18)}  
&  Maine Oct. 2020 (0.2\%)  & 28.85 &  92.07\\
& &  Alabama Jan. 2021 (5.4\%) & 17.87 & 28.57 \\[10pt]

& \multirow{2}{*}{Spouses (0.38)} 
&  Maine Oct. 2020 (0.2\%) & 31.25 &  92.02 \\
& &  Alabama Jan. 2021 (5.4\%) & 19.14 &  27.86 \\
 \hline
\end{tabular}}
%\end{adjustbox}
\footnotesize{Percent increase in sensitivity relative to $H_0$ = $100 *(Sens_{H_a} - Sens_{H_0})/(Sens_{H_0})$; \\ Percent decrease in tests per sample relative to individual testing = $100 * (Tests_{H_a} - n)/(n)$, ($n$=pool size).}
\end{table}



==> COVID Pooled Testing Draft Paper 2/simulations.tex <==
% !TEX root = main.tex

We adapt our simulations in the previous section to account for heterogeneity and uncertainty in $\pi$ and $\tau$ by performing the simulations under three further settings: 
\begin{description}
    \item[Setting 1 - Fixed $\pi$ / Random $\tau$ ](Fixed Prevalence/Random Network Effect): Sample $\tau$ from a Beta prior distribution  and calculate the corresponding probability of $k$ positives due to network transmission. $\pi$ assumed fixed and equal to the point estimate. 
  \item[Setting 2 - Random $\pi$ / Fixed $\tau$] (Random Prevalence/Fixed Network Effect).   Sample $\pi$ from a Beta prior distribution. $\tau$ assumed fixed and equal to the point estimate.
\item[Setting 3 - Random $\pi$ / Random $\tau$ ](Random Prevalence/Random Network Effect): Sample both $\pi$ and $\tau$, as described above.
\end{description}
When sampling $\pi$ and $\tau$, for each point estimate and group size, we perform $B=100$ simulations of sampling from the prior distribution. 
 
 \indent The results of the Monte Carlo simulations for Random $\tau$ and $\pi$ (Random Prevalence/Random Network Effect) are shown in Figure \ref{fig:allmetrics_allgraph}; results for random $\tau$ (Fixed Prevalence/Random Network Effect) and random $\pi$ (Random Prevalence/Fixed Network Effect) are presented in Appendix ~\ref{sec:appendix_sim}, Figures ~\ref{fig:allmetrics_taugraph} and ~\ref{fig:allmetrics_pigraph}. 
 
 These simulations inform the following observation: \\
 \xhdr{Lesson 4} \textit{These findings highlight the importance of developing \textbf{adaptive} pooled testing procedures. With reasonably specified models for prevalence and network transmission, the optimal pool size can be chosen to maximize sensitivity and ensure minimum FDA thresholds are met.  However, even with significant uncertainty and heterogeneity in pools, results are robust. }
 
 \begin{figure}
\includegraphics[width=\linewidth]{Figures/sens_fda_allgraph.png}\hfill
\caption{Proportion of simulated results with sensitivity equal to or greater than the FDA threshold for pooled testing (0.85), using the Random Prevalence/Random Network Effect Model.}
\label{fig:sens_fda}
\end{figure}
 
 In settings with high network transmission (e.g. child index cases, spouses, and household symptomatic index cases), all of the simulation results have sensitivity greater than the FDA threshold for sensitivity (Figure ~\ref{fig:sens_fda}). For low network transmission settings (e.g. healthcare or household asymptomatic index cases), pooled testing with small pools ($n \leq 5$) may still meet minimum FDA standards, but larger pools may not be appropriate (Figure ~\ref{fig:sens_fda}). %Examining the 95\% credible intervals in Figure ~\ref{fig:allmetrics_allgraph} (as well as Figures ~\ref{fig:allmetrics_taugraph} and ~\ref{fig:allmetrics_pigraph}), we see that for settings with high network transmission, even the lower bound of the confidence interval never falls below the FDA threshold for sensitivity. 
 %Comparing Figure \ref{fig:allmetrics_allgraph} and Figure \ref{fig:allmetrics_taugraph}, we see that the heterogeneity in results is primarily driven by uncertainty in $\tau$, not in $\pi$ (see Appendix \ref{sec:appendix_sim} for the results on the Graph Effect). 
 Supporting our previous observations, heterogeneity in results is primarily driven by uncertainty in $\tau$, not in $\pi$. 
 
Additionally, adaptability of the overall model is critical in a pandemic setting, where transmissibility and susceptibility vary over time and space as a function of the particular viral variants circulating and the prevalence of vaccination (and efficacy of vaccines against variants). The simulations presented in this paper can easily be adapted to settings where more transmissible variants are widespread (by increasing the value of the transmission parameter) or as vaccination rates increase (by decreasing the value of the prevalence parameter). The robustness of results to significant uncertainty in parameter values is especially critical in this setting.

 Considering the efficiency of the pooled testing procedure, there is very little variation in expected tests per sample across different specifications of the model and parameters (Figures \ref{fig:allmetrics_allgraph}; Table \ref{table:summary_performance}). In all cases, the pooled sampling procedure results in significant reductions in tests per sample relative to the individual sampling procedure. 



    
 \begin{figure}[H]
    \includegraphics[width=\linewidth]{Figures/combined_allgraph_plots_b.png}\hfill
  \caption{\textbf{Random Prevalence/Random Network Effect Model}: Model-estimated parameters (sensitivity, relative sensitivity, expected tests per sample, missed cases per sample) by pool size, prevalence ($\pi$), and network transmission ($\tau$) when $\pi$ and $\tau$ are sampled from Beta distributions corresponding to the specified scenario. Shaded area indicates the empirical 95 percent credible prediction interval. Proportion of samples with $C_t$ above the 95\% LoD (held constant at LoD = 35) is constant, equal to 25\%. The null (no correlation) model, individual testing, and FDA sensitivity threshold are also indicated, where relevant.}
   \label{fig:allmetrics_allgraph}
\end{figure}




\begin{table}
\caption{Expected performance of pooled testing under select prevalence, network transmission, model type, and pool size scenarios.} 
\label{table:summary_performance}
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1}
%\begin{adjustbox}{width=1.2\textwidth,center}
\resizebox{\textwidth}{!}{\begin{tabular}{@{}ccccccc@{}} 
\hline
\multicolumn{3}{p{3.5cm}}{ }&
\multicolumn{4}{p{8cm}}{\centering \textbf{Model}}\\
 \cline{4-7}
 \multicolumn{3}{p{2.5cm}}{ }&
\multicolumn{2}{p{4cm}}{\centering Random Prevalence/ Fixed Network Transmission}&
\multicolumn{2}{p{4cm}}{\centering Random Prevalence/ Random Network Transmission}\\
 \cline{4-7}
 & Network Transmission ($\tau$)  &Prevalence ($\pi$) & 
 \multicolumn{1}{p{2cm}}{\centering \% Increase Sensitivity \\ Relative to $H_0$}&
\multicolumn{1}{p{2cm}}{\centering \% Decrease Tests/Sample \\ Relative to Individual Testing}&
\multicolumn{1}{p{2cm}}{\centering \% Increase Sensitivity \\ Relative to $H_0$}&
\multicolumn{1}{p{2cm}}{\centering \% Decrease Tests/Sample \\ Relative to Individual Testing}\\
 \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{Pool Size n = 5}} 
& \multirow{2}{*}{Household Asympt. (0.012)}  
& Maine Oct. 2020 (0.2\%) &  0.52 &  79.34 & 0.58 & 79.36\\
%& Oct 2020 & Asympt. (0.012) &   &  &  &  \\  
& & Alabama Jan. 2021 (5.4\%) & 0.50 &  58.77 & 0.53 &  58.92\\[10pt]
% & Jan 2021 & Asympt. (0.012)   &  &  &  & \\  
& \multirow{2}{*}{Household Symptomatic (0.18)}  
&  Maine Oct. 2020 (0.2\%)  & 7.71 &  79.31 & 7.86 &  79.31\\
% & Oct 2020   &Symptomatic (0.18)  &  &  &  &  \\  
& &  Alabama Jan. 2021 (5.4\%) & 7.04 & 58.00 & 7.19 &  57.52\\[10pt]
% & Jan 2021   &Symptomatic (0.18)  &  &  &  &  \\  
& \multirow{2}{*}{Spouses (0.38)} 
&  Maine Oct. 2020 (0.2\%) & 12.8 & 79.28 & 13.09 &  79.27\\
% & Oct 2020    &  &  &  &  &  \\  
& &  Alabama Jan. 2021 (5.4\%) &11.67 & 56.94  & 11.92 &  56.54\\
%& Jan 2021  &  &  &  &  & \\  
 \hline
 
 \multirow{6}{*}{\rotatebox[origin=c]{90}{Pool Size n = 20}}
& \multirow{2}{*}{Household Asympt. (0.012)}  
& Maine Oct. 2020 (0.2\%) & 3.62 &  92.60 & 3.94 &  92.64\\
% &  Oct 2020    & Asympt. (0.012) &  &  &  &  \\  
& & Alabama Jan. 2021 (5.4\%) & 2.55 &  37.74 & 2.71 &  37.12\\[10pt]
% & Jan 2021    & Asympt. (0.012)  &  &  &  &   \\  
& \multirow{2}{*}{Household Symptomatic (0.18)}  
&  Maine Oct. 2020 (0.2\%)  & 28.69 &  92.07 & 28.86 & 92.07\\
%& Oct 2020    &  Symptomatic (0.18)  &  &  &  &   \\ 
& &  Alabama Jan. 2021 (5.4\%) &17.76 &   30.51 & 17.88 &  28.57\\[10pt]
%&  Jan 2021    & Symptomatic (0.18)  &  &  &  &  \\  
& \multirow{2}{*}{Spouses (0.38)} 
&  Maine Oct. 2020 (0.2\%) & 31.17 &  92.03  & 31.20 &  92.02\\
%&  Oct 2020    &  &  &  &  &   \\  
& &  Alabama Jan. 2021 (5.4\%) & 19.09 &  29.70  & 19.11 &  27.87\\
%&  Jan 2021    &  &  &  &  &   \\  
 \hline
\end{tabular}}
%\end{adjustbox}
\footnotesize{Percent increase in sensitivity relative to $H_0$ = $100 \times (\text{Sens}_{H_a} - \text{Sens}_{H_0})/(\text{Sens}_{H_0})$; \\ Percent decrease in tests per sample relative to individual testing = $100 \times (\text{Tests}_{H_a} - n)/(n)$, where $n$=pool size.}
\end{table}











    

==> discussion.tex <==
% !TEX root = main.tex


Pool testing can also be considered as a spectrum: from $p=1$,where we consider individual tests, to $p=\infty$, where we are interested in extremely large pools and in this case, are using pool testing as a monitoring tool (widespread surveillance of the population). In this case , we might not necessarily be interested in the individual samples themselves and perform a two stage Dorfman procedure. Rather, in this section, we investigate how pooled testing can be used as a monitoring tool, and to recover the prevalence level. In particular, we will focus on investigating how PCR can be used quantitatively, rather than qualitatively --- to perform inference.

Suppose that we want to infer the prevalence from group testing.


The probability that the pool tests positive is :
$$ p = 1- (1-\pi)^n $$
We want to infer $\pi$.

If we were to observe $p$ pools the plug in estimator would be:
$$  \bar{Y}_p = 1- (1-\hat{\pi})^n)$$
$$  \hat{\pi} = 1- (1 -\bar{Y}_p)^{1/n} $$

Because we are typically looking at very small probabilities, it might be better to use exact confidence intervals. 

That is, we solve:
$$ \frac{\alpha}{2} \geq \sum_{k=0}^{p\bar{Y}_p} {p \choose p\bar{Y}_p} p_L^{ p\bar{Y}_p} (1-p_L)^{ p- p\bar{Y}_p} \qquad p_L = 1-(1-\hat{\pi}_L)^n$$
$$ \frac{\alpha}{2} \geq \sum_{k=p\bar{Y}_p}^p {p \choose p\bar{Y}_p} p_H^{ p\bar{Y}_p} (1-p_H)^{ p- p\bar{Y}_p} \qquad p_H = 1-(1-\hat{\pi}_H)^n $$

This creates confidence bands that are perhaps a little large (include a plot).


Our other suggestion here is to try to use the quantitative information contained in the Ct value to enrich this. Roughly, if the $C_t$ value is high, it will be more reflective of a low number of samples being positive, and vice versa.

We have:
$$ Y_i = 1\{ C_t \geq T\} $$
Let $m_0$ be the initial quantity of viral material in the initial sample, and $T$ a threshold for declaring the sample as positive:
$$ m^{(0)} 2^{C_t} = T \implies m^{(0)} =  \frac{T}{2^{C_t}} $$
Thus, in the combined sample:
$$ M = \sum_{i=1}^n m^{(0)}_i =  \sum_{i=1}^n \frac{T}{2^{C^t_i}} $$
$$ \implies C_M^t = \frac{\log( \frac{T}{ \sum_{i=1}^n \frac{T}{2^{C^t_i}}})}{\log 2} = \frac{-\log( \sum_{i=1}^n \frac{1}{2^{C^t_i}})}{\log 2} $$


So we transform the problem of inferring the prevalence in:

$$ \text{Find $\pi$ such that: }\qquad \pi = \tetx{argmax}_{\pi} \ell(\pi)  $$

(MLE) of the latent variable model, with:
$$  C_i \sim  \text{Mixture}(0, \text{Weibull) with probability $\pi$} $$
We can probably provide an abacus of sorts: We can get via MCMC simulations the distribution of $C_M^t$for different numbers of positives. And treat $\pi$ as Bernouilli (makes sense for very large pools), and:
\begin{itemize}
    \item We look at all the distributions of $C_M$ that overlap with the observed value (probability of observing that value between $[2.5;97.5]$).
    \item We use the min and max values of the prev of these distributions to infer what the prevalence is.
\end{itemize}

The issue with this procedure is that it is based on a discretization of the space. So it might require a lot of computations? Remains to show that this yields better result than the naive binomial way of doing things. Let's do simulations to check.
